ParaCell: Paravirtualized Secure Containers with Lightweight Intra-Container Isolation and Intent-Driven Memory Management

Secure containers isolate each container with its own kernel, mitigating shared-kernel attacks prevalent in traditional container systems. However, existing designs still face a fundamental isolation--performance trade-off. Nested-cloud deployments amplify the cost of VM exits and page-table management, while emerging agentic workloads expose bursty memory demand that requires fine-grained elasticity. We attribute this trade-off to two root causes. First, existing designs lack lightweight intra-container isolation primitives for frequent container user--kernel transitions. Second, the host treats container memory management as opaque, forcing reactive secondary faults and coarse-grained huge page mappings to amortize their cost. This paper presents ParaCell, a paravirtualized secure container runtime built on two insights. First, intra-address-space hardware protection primitives can provide lightweight intra-container isolation. ParaCell uses MPK-based XGates to isolate the container user and container kernel within a single address space, turning frequent user--kernel transitions into direct domain switches. Second, container kernel allocators already encode memory-management intent. ParaCell introduces Pager to interpose on allocation and free events, batch proactive GPA to HPA bindings and unbindings, and avoid reactive shadow page-table faults while preserving fine-grained memory elasticity. ParaCell is implemented as a drop-in replacement for RunV. Our experiments demonstrate that, across traditional cloud and emerging agent applications, ParaCell reduces latency by up to 57% and 79% over PVM, and by up to 33% and 88% over RunV, in bare-metal and nested setups, respectively. On agent workloads, ParaCell saves up to 35.6% memory compared with the state-of-the-art VM memory reclamation technique, HyperAlloc.

==> Makefile <==
NAME=paper
all:  $(NAME).pdf

BASE := Makefile $(wildcard *.tex) $(wildcard *.bib)
BASE := $(BASE) $(shell find ./figures -name '*.eps')
# Do not add $(shell find ./figures -name '*.svg'): Make splits prerequisites on
# spaces, so SVG paths containing spaces become invalid targets and break the
# paper.pdf rule. Rebuild after editing SVGs via touching paper.tex or `make clean`.
BASE := $(BASE) $(shell find ./plots -name '*.eps')

%.pdf:  %.tex $(BASE)  acmart.cls ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev -shell-escape $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev -shell-escape $(notdir $<)
	cd $(dir $@) && pdflatex-dev -shell-escape $(notdir $<)
#	if ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
#	  then cd $(dir $@) && pdflatex-dev $(notdir $<); fi



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	$(NAME).pdf $(NAME).xcp $(NAME).fdb_latexmk $(NAME).fls


clean: docclean

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> design_deprecated.tex <==
\section{Detailed Design}
\label{sec:design}

% Swift Switch Gates

% \begin{figure*}[htbp]
%     \centering
%     \subfloat[Lightweight Switches within \gates{}]{%
%         \begin{minipage}[b]{0.49\textwidth}
%             \centering
%             \includesvg[height=0.18\textheight]{figures/gates}
%             \label{fig:design:gates}
%         \end{minipage}}%
%     \hfill
%     \subfloat[Race suppression mechanism]{%
%         \begin{minipage}[b]{0.49\textwidth}
%             \centering
%             \includesvg[height=0.18\textheight]{figures/ctrcall}
%             \label{fig:design:ctrcall}
%         \end{minipage}}
%     \caption{Layout of switch gates and race suppression mechanism.}
% \end{figure*}

\subsection{Lightweight Intra-container Isolation}

Intro-container isolation necessitates the implementation of privilege transitions, or domain switch, within the container.
Prior work ~\cite{huang2023pvm}~ has already adopted vcpu-level state sharing (control registers, event vector, stack pointer, etc.), noted as paravirtualized
vcpu control structure (PVCS) to paravirtualize the privilege transition. Such a design retains the software semantics of
the domain switch, but introduces full world switch with the host under each occurence. Leveraging protection keys to complement the current style of privilege transitions
for kernel separation underscores the need to redesign the routine trampolines to perform critical paravirtualized switches in specific call sites. 
The key challenge is to swiftly and faithfully preserve both spftware semantics, and more importantly, the hardware semantics on the guest domain switch path. 
To achieve this, we hereby present the design of \gates{} mechanism.

\stitle{Overview of \gates{}} Figure~\ref{fig:design:gates} sketches the gate layout, including the syscall gate and the event delivery gate.
The syscall gate runs in ring~3 so that common syscalls can invoke guest-kernel handlers directly instead of relying on host-side emulation.
The event-delivery gate runs in ring~0 to implement a fast path for delivering events to the guest kernel (and related control transfers) with minimal host-side emulation.
On the container side, we partition the unified guest address space into GU and GK: MPK distinguishes executable GK text from non-executable non-read-writable regions so that GU cannot 
enter the kernel except through designated gates. In between the two gates, Guest-Host shared PVCS are also mapped into the \gates{} to maintain the correct hardware semantics on the critical section.
Any lightweight switch (e.g., syscall, event delivery) between GU and GK
must use these lightweight switch gates to perform the correct MPK switch to the corresponding memory domain, or resolve to the full world switch with the host.
As \emph{wrpkru} instruction shall only reside in two corresponding switch gates,
we use previously developed state-of-art binary rewriting techniques in prior work ~\cite{vahldiek2019erim} to remove the corresponding instructions from 
the original binary and add special state checksbefore effective routines are called to mitigate potential ROP attacks.
\gates{} also drops the costly IBRS and KPTI as weremove the shared host-kernel mappings from the guest address space except for the PVCS data structure as it is considered private
on the guest container side.
\begin{figure}[htbp]
    \centering
    \includesvg[width=\columnwidth]{figures/gates}
    \caption{Lightweight switches within \sys{} container via \gates{}. EVGate: Event Gate. Ctr-Call: Morphed Syscall Invocation.}
    \label{fig:design:gates}
\end{figure}

\iffalse
\stitle{Reengineering Address Space} Lightweight switches require a single address space: we merge the previously distinct spaces into one unified layout and repartition it with distinct permissions.
This is non-trivial because the host kernel and guest kernel may install \emph{conflicting} identity mappings on the same physical page table.
We therefore use a position-independent guest kernel (\emph{PIE kernel}) that relocates its identity mapping, based on its designated CPU id, to a canonical region at startup.
With that layout in place, we subdivide the unified space with Memory Protection Keys (MPK) for fine-grained isolation.
On the container side we partition GU and GK: MPK distinguishes executable GK text from non-executable regions so that GU cannot enter the kernel except through designated gates.
On the host side we similarly partition container-controlled and host-controlled mappings under MPK so that the container cannot execute host kernel code except through gates.
Similarly, we add the corresponding \emph{wrpkrs} instruction in the corresponding redirection site to preserve the compatibility.
\fi

\stitle{Ctr-Gate} To reduce the frequency of host mediation on common syscall paths, we observe that the performance-critical syscall set
is small and typically follows stable calling conventions with limited semantic variation. In this sense, such privilege calls
can be seeminglessly transformed into a direct functional invokation (we refer as \emph{ctr-call} and \emph{ctr-ret}) plus two lightweight switch to the guest kernel. Building on the latest syscall rewriting techniques\cite{yasukata2023zpoline},
we exhaustively rewrite the syscall sites on the during load time and inject the trampoline to the corresponding per application thread syscall site on the fly.

After the loader patches the syscall site, at runtime the application jumps to a syscall trampoline that validates the syscall number and arguments and
decides whether direct execution of the guest-kernel handler is safe.
On the \emph{ctr-call} path, the trampoline relayes to the switch gate and invokes \emph{to\_kernel} function to perform a world switch.
During the word switch, the gate switches to the guest-kernel memory domain, moves to the guest-kernel stack, sets the correct \emph{kernel\_gs} pointer,
builds the syscall frame, and invokes the handler. On \emph{ctr-ret}, the syscall routine falls back to the \emph{ctr-ret} trampoline then issues
another world switch on \emph{to\_user} function, which restores the prior context on the kernel stack and
switches back to the guest user memory domain before resuming GU execution. The mechanism remains opt-in: sensitive syscalls can bypass rerouting when stronger isolation semantics are required.

\stitle{Interrupt-in-switch Problem} This design however introduces two key challenges to resolve. First, the ctr-gate must mitigate interrupt-in-switch races that can corrupt transient gate state. In the legacy redirection path, this race is avoided by a hardware guarantee 
(\emph{syscall} on x86 disables interrupts at entry). However, some paravirtualization frameworks, such as PVM, require mandatory interrupt delivery during guest-user execution, 
so the gate needs an explicit mechanism to suppress event delivery on the vCPU thread while the gate is executing. 
Second, the syscall gate must retrieve the correct kernel stack pointer and \emph{kernel\_gs} pointer from the PVCS data structure. 
Only the current PVCS is valid at syscall time but not visible on the \gates{} view point; a pre-assigned virtual PVCS pointer (VPVCS) at initialization time=
cannot safely index the context because guest-side thread migration may occur between syscall entry and PVCS context switch.

To ensure correct per-vCPU context lookup, the syscall gate registers its VPVCS pointer at thread granularity with the guest kernel
during gate initialization and introduces an exit-work flag to signal possible thread migration. If migration is detected, guest-kernel exit work remaps the vPVCS to the new physical PVCS position. 
To close the remaining race window during gate execution with a grace period of just single instruction, we add an interrupt-shadow bit in the PVCS control structure. 
The syscall gate sets this bit on entry and clears it on exit; each operation is a single instruction. 
This mechanism suppresses interrupt delivery during the critical section and prevents races that could corrupt transient gate state.
Figure~\ref{fig:design:ctrcall} sketches the race suppression mechanism.
\begin{figure}[htbp]
    \centering
    \includesvg[width=\columnwidth]{figures/ctrcall}
    \caption{Interrupt-in-syscall suppression mechanism. virq cannot be injected into if shadow bit is set.
PVCS: Paravirtualized vCPU Control Structure. virq: Virtual Interrupt Request.}
    \label{fig:design:ctrcall}
\end{figure}
To prevent arbitrary guest-application modification of the control structure, 
we protect the PVCS context-pointer mapping and guest-kernel space with MPK, 
limiting modifications to the syscall gate and the guest kernel.

\stitle{Event Gate} To reduce the latency of event delivery on VM-Exit, 
the key observation is similar to the syscall gate. Major performance-critical events are typically small and predictable
in secure container workloads such as page faults. These events do not require deep interaction with complicated
logics, thus can be preempted in the fast path to bypass the heavyweight host-side emulation path.

We introduce the event delivery gate to bridge the host-side event delivery path to the guest-side delivery path. During VM-exit, the guest will first
traps into the designated entry that is recorded inside the event gate's IDT (Interrupt Descriptor Table) to perform the necessary checks.
The gate will first checks the interrupt vector and decides whether to issue full host emulation. On page fault event, 
the gate will quickly retrieves and injects the page fault to the host without any host-side emulation. As heavy-weight host-side domain switches are optimized out, 
the latency is greatly reduce on critical path.

To reduce event-return latency, we use a compact return event gate that restores guest user execution safely with low latency.
On return, the guest kernel prepares a specialized context frame with the guest return instruction pointer and stack pointer. Because the guest kernel runs at ring~3 in this model, 
it cannot perform the privilege transition itself (e.g., via \emph{iret}). It therefore issues a dedicated switch call that requests gate-mediated return routine.
The return gate temporarily switches to host owned \emph{host\_gs} to access the control structure to check the potential pending interrupt. If not, it 
validates address bounds and audit the \emph{rflags} constraints before transfers control to the guest. By avoiding heavyweight host-side context switches and minimizing
host intervention, this path substantially outperforms the conventional return path.

\subsection{Fine-Grained Elastic Memory Management}
\label{sec:mem}

\stitle{Identifying guest memory management intent.}
Traditional virtualization virtualizes the MMU and page table abstraction.
However, this abstraction does not reflect actual memory usage:
a guest kernel typically establishes an identity mapping (or a fixed-offset direct mapping) that covers its entire GPA range at boot time,
so all guest page-table entries are populated long before any page is actually used by a workload.
The hypervisor, treating the guest as an opaque process, cannot distinguish a pre-mapped but idle page from one actively in use,
and must therefore fall back to on-demand paging via secondary faults to discover actual access patterns.

The guest kernel's page allocator provides the missing signal.
A physical page enters active use only when the allocator hands it out and becomes reclaimable only when the allocator takes it back.
These allocation and free events precisely indicate when a GPA requires, or no longer requires, a backing host physical page.
By exposing these events to the host instead of virtualizing MMU and page table operations,
\sys{} can bind a GPA to an HPA at allocation time and unbind it at free time,
replacing reactive, fault-driven two-stage translation with proactive, intent-driven single-stage translation.

\stitle{Explicit GPA$\rightarrow$HPA (un)binding.}
To realize this intent-driven model, \sys{} introduces the \pager{}:
a dedicated memory mediator that translates guest allocation/free operations into GPA$\rightarrow$HPA bindings/unbindings on host pages.
% Conceptually, the hypervisor exposes an exokernel-like memory interface:
% it retains ownership of host physical pages and manages guest memory as discrete host pages,
% while the guest kernel continues to operate over a conventional contiguous GPA space,
% with the \pager{} translating between GPA and HPA.
%
To handle the pre-mapped direct mapping,
the guest explicitly registers this region with the \pager{} so that these PTEs are managed according to allocator lifecycle events rather than their static presence.
Figure~\ref{fig:design:pager} illustrates the workflow for page allocation and free, as well as page table updates.

On allocation (green color in the figure), the \pager{} (1)(4) (as explained later) allocates a backing page from the host, (2) records the GPA$\rightarrow$HPA binding.
It also immediately (3) maps the translated HPA into the direct-mapping PTE,
as this allocation typically indicates that the guest kernel will soon access the page through the direct mapping,
for example to clear the page or populate it with file data (e.g., page cache).
On subsequent mappings (blue color) of the same GPA (e.g., into user-space page tables),
the guest kernel first (1) calls \texttt{get\_free\_pages} to obtain the page,
after which the \pager{} (2) looks up the corresponding HPA and (3) installs it into the hardware-walked page table,
eliminating further secondary faults.
When a guest page is freed (orange color), the \pager{} performs the reverse:
it (2) revokes the binding from the table, (3) removes the direct mapping
and (1)(4) (as explained later) returns the backing host page to the hypervisor.
This keeps host-allocated memory tightly aligned with guest usage at 4KB granularity,
avoiding the inefficiencies of coarse-grained mechanisms such as ballooning,
hotplug, and delayed host-side reclamation.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\columnwidth]{figures/pager.eps}
    \caption{\pager{} architecture and workflow. PT: page table. DM-PT: page table managing direct mapping. GFP: \texttt{get\_free\_pages}. Iso: Isolation.}
    \label{fig:design:pager}
\end{figure}

\stitle{Enprivileged \pager{}.}
The isolation boundary of the \pager{} is a key design choice to further reduce per-switch overhead.
Isolating it inside the hypervisor would force every mediated operation to cross the expensive guest--host boundary.
Conversely, isolating it within a conventional guest component is insufficient,
as page table updates and TLB maintenance are privileged operations.
\sys{} therefore colocates \pager{} with the guest kernel in the same address space but enprivileges it to the kernel mode,
separating them only by user/kernel privilege levels.
Privilege-level isolation is sufficient,
as the \pager{} maintains only per-VM private state and contains no global data.
By avoiding shared host-kernel mappings,
switching to \pager{} does not require side-channel mitigations such as KPTI and IBRS.

\stitle{Pre-binding and deferred unbinding on PCP lists.}
The remaining cost is host page handoff between the hypervisor and the \pager{}.
If each allocation and free operation triggers an immediate bind or unbind,
the design still incurs frequent full context switches to the host.
Hence, \sys{} piggybacks on Linux per-CPU page (PCP) lists,
which serve as a per-core cache between the fast allocation path and the global buddy allocator.
PCP lists allow most allocations and frees to be handled locally without touching global allocator,
and only refill from or drain back to the buddy allocator in batches.
It was designed to reduce contention on the global allocator and avoids cross-CPU cacheline bouncing.

Specifically, pages in the global buddy allocator remain unbound and have no backing HPA.
Binding and unbinding happen at the boundary between PCP lists and the buddy allocator.
As shown in Figure~\ref{fig:design:pager},
when a PCP list is refilled (orange color in the figure) from the buddy allocator,
the \pager{} obtains a batch of host pages from the hypervisor and pre-binds them to the corresponding GPAs;
when pages drain (green color) from a PCP list back to the buddy allocator,
the \pager{} unbinds the batch and returns the host pages.
Individual allocations (e.g., \texttt{get\_free\_pages}) and frees on the hot path merely move pre-bound pages in and out of PCP lists without any host involvement.
This preserves the mature low-contention PCP design,
minimizes intrusive allocator changes, and keeps elasticity off the hot path.
Meanwhile, the memory overhead of pre-bound but not-yet-allocated pages is negligible,
as the size of a single PCP list is typically small, accounting for less than 1\% of total memory.

\iffalse
\subsection{EBPF-guided Delivery and Notification}

Virtualizing interrupt delivery and notification in secure containers suffers from three recurring bottlenecks: 
(1) multi-stage interrupt handling that repeatedly crosses guest--host protection boundaries, 
(2) frequent CR3/page-table switches that increase TLB disruption, and
(3) heavy virtio/vhost scheduling overhead under high I/O concurrency. Together, these effects inflate tail latency and reduce throughput on the common I/O path. We address these bottlenecks with two complementary mechanisms: eBPF-guided event delivery for host-to-guest fast paths, and selective device-emulation bypass for guest-to-host virtio operations.

\stitle{EBPF-guided Event Delivery (H -> G)}
To reduce interrupt latency, we exploit the fact that secure containers typically rely on a small, predictable interrupt set: timer interrupts (scheduling), page-fault interrupts (memory management), and virtio interrupts (device I/O). These cases often do not require deep interaction with complex host emulation paths.
Motivated by recent eBPF-based fast-path designs, we build an eBPF-guided delivery layer that bridges host-side gates and KVM injection paths. Each performance-critical interrupt is bound to an eBPF handler that decides, at interrupt time, whether to inject directly into GK or forward to the host kernel for full processing.

For timer interrupts, the eBPF program consults sched-ext state to determine whether the source corresponds to guest or host timer activity.
For page faults, the eBPF logic performs guest page-table translation checks to distinguish guest-mapping faults from host-managed cases.
For virtio interrupts, eBPF maps are used to notify the corresponding entry gate and trigger direct guest-side handling.
To further reduce \texttt{irqfd}-induced latency between virtio signaling and guest execution, sched-ext is used to prioritize the target vCPU thread immediately after interrupt issuance and injection.

To reduce CR3 switch frequency and associated TLB penalties, we mirror host-kernel identity mappings into a protected guest shadow page table and guard that table with MPK.
On the fast path (directly deliverable events), no CR3 switch is needed.
On the slow path (events requiring host processing), execution switches to the host-kernel page table and continues through the regular delivery path.
This design preserves a low-latency fast path for common events while retaining compatibility through the slow path.

\stitle{Device Emulation Bypass (GK -> H)}

To reduce the overhead of emulation and notification stack, we introduce a gated emulation-bypass path for common virtio operations.
When safety checks and queue state permit, GK can publish descriptors and consume completions through a narrow, pre-validated gate interface that bypasses the full host-emulation slow path.
When vhost-kernel is possible, we select the inline model for tx packet processing. By offloading the packet processing directly in the vcpu thread context,
we eliminate the need to switch to the vhost-thread, bypassing the cost of vhost-thread context switch. On the rx path, we delegate the packet
processing to a series of vhost-kernel threads, to maximize the parallelism.


Fallback to the regular host path remains mandatory for unsupported operations, malformed descriptors, or policy-sensitive cases, preserving compatibility and isolation.
This selective bypass shortens the I/O critical path while maintaining a conservative correctness envelope.
\fi


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> security-analysis.tex <==
\section{Security Analysis}
\label{sec:security-analysis}

